Synchronization of Micromechanical Oscillators Using Light

Synchronization, the emergence of spontaneous order in coupled systems, is of fundamental importance in both physical and biological systems. We demonstrate the synchronization of two dissimilar silicon nitride micromechanical oscillators, that are spaced apart by a few hundred nanometers and are coupled through optical radiation field. The tunability of the optical coupling between the oscillators enables one to externally control the dynamics and switch between coupled and individual oscillation states. These results pave a path towards reconfigurable massive synchronized oscillator networks.

==> synchronization_main_text_arxiv.tex <==
% !TEX root = sync_arXiv.tex

Synchronization processes are part of our daily experiences as they occur widely in nature, for example in fireflies colonies~\cite{BucBuc6803}, pacemaker cells in the heart~\cite{Pes75}, nervous systems~\cite{WhiTraJef9502} and circadian cycles~\cite{Str03}. Synchronization is also of great technological interest since it provides the basis for timing~\cite{Ngu0702}, navigation~\cite{Bah09}, signal processing~\cite{Bre02}, microwave communication~\cite{CuoOpp9307}, and could enable novel computing~\cite{MahYam0805,BliQinKim0707} and memory concepts~\cite{AonKurOka9903,BagPooLi1110}. At the micro and nanoscale, synchronization mechanisms have the potential to be integrated with current nanofabrication capabilities and to enable scaling up to network sizes. The ability to control and manipulate such networks would enable to put in practice nonlinear dynamic theories that explain the behaviour of synchronized networks~\cite{Str98,HopIzh0102,Mar1110}. Recent work on coupled spin torque~\cite{KakPufRip0509,ManRizEng0509} and nanoscale electromechanical oscillators (NEMS)~\cite{ShiImbMoh0704,ZalAubPan0310} exhibit synchronized oscillation states. However, the major challenges with synchronized oscillators on the nanoscale are neighbourhood restriction and non-configurable coupling which limit the control, physical size and possible topologies of complex networks~\cite{HeiLudQia1107,MarHarGir0603,Mar1110}. Here, we demonstrate the synchronization of two dissimilar silicon nitride (Si$_3$N$_4$) optomechanical oscillators coupled only through optical radiation field as opposed to the traditional coupling through physical contact. The tunability of the optical coupling between the oscillators enables one to externally control the dynamics and switch between coupled and individual oscillation states. These results pave a path towards realizing massive synchronized oscillator networks.
\begin{figure}
\begin{center}
\includegraphics[scale=1,angle=0]{fig_main1_single_column_arxiv.pdf}
\caption{Design of the optically coupled optoemchanical oscillators (OMOs).  (\textbf{a}) Schematic of the device illustrating the mechanical mode profile and the optical whispering gallery mode. (\textbf{b}) Scanning electron micrograph (SEM) image of the OMOs with chrome heating pads for optical tuning by top illumination. (\textbf{c},\textbf{d}) The symmetric (S) and anti-symmetric (AS) coupled optical supermodes. The deformation illustrates the mechanical mode that is excited by the optical field. (\textbf{e}) The dynamics of the coupled OMOs can be approximated by a lumped model for two optically coupled damped-driven nonlinear harmonic oscillators.}
\label{fig:fig1main}
\end{center}
\end{figure}

In optomechanical oscillators (OMOs) the mechanical oscillations can be controlled by light. These structures support tightly confined optical modes as well as long-living (high quality factor) mechanical vibrational modes \cite{KipVah07,LinRosJia0905}. When an optical resonance is excited, both light and sound become localized within the cavity's small volume, which leads to a strong coupling between the optical and mechanical fields. The optical modes are affected by the geometric distortions induced by the mechanical modes and the mechanical modes are affected by forces on the structure exerted by the optical modes. This mutual feedback between light and sound, proposed first in the context of gravitational wave detectors~\cite{BraStrVya0109}, has been explored to amplify or cool down mechanical modes of mesoscopic structures~\cite{ArcCohBri06}. Recent work shows that when such feedback is negative, cooling of the mechanical mode to its quantum mechanical ground-state can be achieved~\cite{ChaAleSaf1110,NaiBuuLaH0609,SchArcRiv0907,Gro09}. When operating the optomechanical cavity in the positive feedback regime, the optical mode provides gain to the mechanical mode. Above a certain threshold power, when the gain is high enough to overcome the intrinsic mechanical damping, the mechanical mode starts a regenerative oscillation and behave as a free-running oscillator. The transmitted laser signal becomes deeply modulated at the mechanical frequency of the oscillator~\cite{CarRokYan05,KipVah07,GruLeePai1002}. We demonstrate here that when two such OMOs are fabricated with slightly different dimensions (i.e. slightly different mechanical frequencies) and are coupled through the optical field, the two OMOs can achieve synchronization. By switching off and on of the optical coupling between two OMOs we demonstrate that both the individual free-running and synchronized oscillation dynamics can be achieved.

Each individual OMO, shown in figure  \hyperref[fig:fig1main]{\ref{fig:fig1main}a,b} consists of two suspended vertically stacked Si$_3$N$_4$ disks with high optomechanical coupling~\cite{WieCheGon0912,WieManLee1101,LinRosJia0905,RosLinPai0908}. They are fabricated using standard e-beam lithography followed by dry and wet etching steps [see supplementary information (SI)]. The two disks are $40$~\textmu m in diameter and $210$~nm in thickness while the air gap between them is $190$~nm wide. Such a small gap and the relative low refractive index of Si$_3$N$_4$ ($n \approx 2.0$) induce a strong optical coupling between the top and bottom disks. Since the optical modes of the stacked disks depend strongly on their separation, any mechanical mode that modulates the vertical gap induces a corresponding modulation in the optical resonant frequency; a measure for the efficiency of this process is the optomechanical coupling, defined as ${g_{om}} = \partial \omega /\partial x$ where $\omega $ is the optical frequency and $x$ is the mechanical displacement amplitude. In our device this is calculated to be $g_{om}/2\pi =49$~GHz/nm (see SI). The mechanical mode that couples most strongly to the optical field is also illustrated by the deformation in figure \hyperref[fig:fig1main]{\ref{fig:fig1main}a} which has a natural frequency of ${\Omega _m}/2\pi  \approx 50.5$~MHz.

In contrast to most micro-scale synchronization demonstrations, the two OMOs are not physically connected, instead they are separated by a distance of ${d_g}=(400\pm20)$ nm. Due to the evanescent optical coupling between the left ($L$) and the right ($R$) OMOs, optical supermodes are formed with a spatial profile that spans both the $L$ and $R$ cavities (see fig. \hyperref[fig:fig1main]{\ref{fig:fig1main}c,d}). The resulting optical resonance splits into a symmetric, lower frequency mode (fig. \hyperref[fig:fig1main]{\ref{fig:fig1main}c}) and an anti-symmetric higher frequency mode (fig. \hyperref[fig:fig1main]{\ref{fig:fig1main}d}). Light coupled to any of these supermodes interacts with both the $L$ and the $R$ cavities and therefore we can choose to pump light only into one of the cavities (through a taper fibre); we choose the $R$ OMO, as shown in the schematic of figure \hyperref[fig:fig2main]{\ref{fig:fig2main}a}. As light interacts with the $R$ OMO above its oscillation threshold, it excites the OMO to a regenerative oscillation mode which in turn induces modulation of the light at its mechanical frequency ${\Omega _R}$. When light tunnels through the gap to interact with the $L$ OMO, it forces the left cavity with resonant frequency ${\Omega _L}$ to entrain into the right cavity frequency ${\Omega _R}$; the reciprocal occurs when light interacts back with the $R$ OMO. This mutual injection of the modulated light from the two OMOs form the basis for entrainment and the onset of synchronized oscillation~\cite{CroZumLif0411,HolMeaMil1105} (see SI for details).
\begin{figure*}
\begin{center}
\includegraphics[width=0.9\textwidth,angle=0]{fig_main2_arxiv.pdf}
\caption{Controlling the two OMO system. (\textbf{a}) Schematic of the experimental setup. The pump and probe light are launched together into the cavities and are detected separately by photodiodes (PD). An erbium doped fibre amplifier (EDFA) is used to amplify the transmitted signal to increase the signal strength. (\textbf{b}) Transmission spectrum of the coupled cavities. The green and orange coloured optical resonances correspond to the pump and probe resonances respectively. NT: normalized transmission. (\textbf{c}) Anti-crossing of the optical mode as the relative temperature of the $L$ OMO ($T_L$) and the $R$ OMO ($T_R$) is changed through varying the tuning laser power. The tuning laser is focused on to the two OMOs respectively to obtain the negative and positive relative temperatures. (\textbf{d}) Transmission spectrum of the maximally coupled state indicated by the white horizontal line in (c).}
\label{fig:fig2main}
\end{center}
\end{figure*}

We control the degree of optical coupling between the $L$ and $R$ OMOs by thermo-optic tuning of the optical resonant frequencies. Note that the maximum optical coupling between the two OMOs is also limited by the gap size between them (${d_g} = (400\pm20)$ nm). This limitation however can be overcome by connecting the cavities with optical waveguides~\cite{ManWeiLip11}. In our device, as illustrated in the schematic of figure \hyperref[fig:fig2main]{\ref{fig:fig2main}a}, the tuning of optical frequencies is accomplished using an out-of-plane laser beam with wavelength 1550 nm, that can be focused on either OMO. In the center of both OMOs we deposit a 200 nm layer of chrome in order to  increase the heating efficiency of the laser (see fig. \hyperref[fig:fig2main]{\ref{fig:fig2main}a,b}); in our experiment we chose to tune the $L$ OMO which is not directly coupled to the tapered fibre. As heat is dissipated in the chrome pads, the cavity temperature increases which in turn red shifts the optical resonance of the cavity through the thermo-optic effect~\cite{ArmMinMar0411}. A signature that the optical frequency of both OMOs is matched is given by the almost symmetric resonance dips observed in the optical transmission spectrum (fig.  \hyperref[fig:fig2main]{\ref{fig:fig2main}b} and \hyperref[fig:fig2main]{\ref{fig:fig2main}d}). The degree of optical coupling between the oscillators can be controlled by the heating laser power (fig. \hyperref[fig:fig2main]{\ref{fig:fig2main}c}). We are able to both either maximize the coupling or completely decouple the two OMOs (see SI). 

Individual characteristics of the two OMOs are measured separately by switching off the coupling and exciting the optical modes of each cavity with a continuous wave (CW) laser coupled to a tapered optical fibre. As the laser frequency is swept (from a higher to a lower frequency) across the optical resonance of the OMOs, the radio-frequency (RF) spectrum of the transmitted laser signal is detected by the photodiode (PD) and recorded using a RF spectrum analyser (RSA). The results revealing the single-cavity optomechanical dynamics are shown in figure \hyperref[fig:fig3main]{\ref{fig:fig3main}a,b}. Due to the optical spring effect~\cite{WieManLee1101,SheGraMow0405}, the natural mechanical frequencies $(f_L,f_R)=(\Omega _L,\Omega_R)/2\pi=(50.348,50.237)$~MHz  increase whereas the intrinsic mechanical damping is reduced. The intrinsic mechanical quality factors of the two OMOs are $(Q_{m_L},Q_{m_R})=(2.3\pm0.2,3.4\pm0.3)\times 10^3$. Above a specific laser-cavity detuning, indicated by the horizontal white dashed lines on figure \hyperref[fig:fig3main]{\ref{fig:fig3main}a,c} the mechanical losses are completely suppressed by the optomechanical gain and the OMO enters a regenerative free-running oscillation mode, characterized by sudden linewidth narrowing and amplitude growth. This behavior have been theoretically shown to be a Hopf bifurcation of the optomechanical oscillator~\cite{HeiLudQia1107,MarHarGir0603,HolMeaMil1105}. The lower amplitude peak before the bifurcation is due to amplified thermal Brownian motion of the cavity mechanical mode. It is clear that each cavity has only one mechanical mode in the frequency range of interest. Due to the slight difference in geometry, these frequencies differ by $\Delta f  = f_L - f_R  = (70.0\pm0.5)$~kHz.

We show the onset of synchronization by sweeping the pump laser across the optical resonance, analogously to the single-cavity measurements. This is performed at various power levels, starting from slightly above the estimated oscillation threshold power of the $L$ and $R$ OMOs, ${P_{th - (L,R)}} \approx (640,880)$~nW, up to several times the threshold power (see SI). Using the heating laser, we also tune the optical coupling to its maximum value, indicated by the dashed-white line in figure \hyperref[fig:fig2main]{\ref{fig:fig2main}c}.  At a relative low input power, ${P_{in}} = (1.8\pm0.2)~$\textmu W, the mechanical peaks at $f_R$ and $f_L$ are simultaneously observed  on the RF spectrum shown in figure \hyperref[fig:fig3main]{\ref{fig:fig3main}c}, below the dashed-white line. When the laser frequency is closer to the optical resonant frequency, a Hopf bifurcation occurs and both OMOs start to oscillate. Since cavity $R$ has a higher oscillation threshold, due to its lower mechanical quality factor, it requires more optical power and therefore oscillates closer to the optical resonance. At a higher input optical power level, ${P_{in}} = (11\pm1)$~\textmu W, shown in figure \hyperref[fig:fig3main]{\ref{fig:fig3main}d}, the first Hopf bifurcation takes place at $\Delta {\omega _L}/2\pi  \approx - 0.10$~GHz, and similarly to the case shown in figure \hyperref[fig:fig3main]{\ref{fig:fig3main}c}, the $L$ OMO oscillates first. However, as the laser frequency further moves into the optical resonance, the two OMOs start oscillating in unison at an intermediate frequency of $f_S={\Omega _S}/2\pi  = 50.37$~MHz, which is a clear sign of synchronization. At even higher optical input power, ${P_{in}} = (14\pm1)$~\textmu W, the OMOs do not oscillate individually and instead go directly into synchronized oscillation after the white-dashed line in figure \hyperref[fig:fig3main]{\ref{fig:fig3main}e}. 
\begin{figure*}[htbp!]
\begin{center}
\includegraphics[width=\textwidth,angle=0]{fig_main3_arxiv.pdf}
\caption{RF spectra of the OMOs and synchronization (\textbf{a}, \textbf{b}) RF power spectra of cavity $L$ (a) and $R$ (b) as a function of laser frequency when the coupling is turned off.  The horizontal white lines indicate the onset of self-sustaining oscillation.  PSD: power spectral density. (\textbf{c}) When the coupling is turned on, at an input power $P_{in}=(1.8\pm0.2)$~\textmu W cavities $L$ and $R$ do not synchronize and oscillate close to their natural frequencies (see SI). (\textbf{d}) At ${P_{in}}=(11\pm1)$~\textmu W synchronization occurs after the horizontal solid white line. The synchronized frequency appears between the two cavities natural frequencies but only appear after a region of unsynchronized oscillation (between the dashed and solid white lines). (\textbf{e}) The system oscillate directly in a synchronized state at input optical power ${P_{in}}=(14\pm1)$~\textmu W. (\textbf{f},\textbf{g},\textbf{h}) Corresponding numerical simulations for the OMO system based on the lumped harmonic oscillator model illustrated in fig. \hyperref[fig:fig1main]{\ref{fig:fig1main}d}. NPSD: normalized power spectral density.}
\label{fig:fig3main}
\end{center}
\end{figure*}

To confirm that the OMOs are synchronized we performed numerical simulations for each of the power level we tested based on the experimentally measured mechanical, optical frequencies and quality factors. We calculated the effective motional mass $m_{eff}$ and the optomechanical coupling $g_{om}$  from finite element simulations (FEM). The dynamics of the coupled OMOs is described by a lumped model for two damped-driven nonlinear harmonic oscillators that are optically coupled and experience thermal noise (see SI). The simulated spectra in figure \hyperref[fig:fig3main]{\ref{fig:fig3main}f,g,h} exhibit all the essential dynamics and show good agreement with the corresponding measured spectra.
 
\begin{figure*}[htbp!]
\begin{center}
\includegraphics[width=0.9\textwidth,angle=0]{fig_main4_arxiv.pdf}
\caption{Pump-probe measurement of the individual OMOs oscillation when coupled. The input pump power is $P_{in} = (11\pm 1)$~\textmu W as in fig. \hyperref[fig:fig3main]{\ref{fig:fig3main}d}. (\textbf{a},\textbf{b}) Schematic of the pump-probe measurement principle. While the pump laser (green) is symmetrically shared between the two OMOs, the probe laser (blue for probing $R$ and red for $L$) can measure each cavity selectively. (\textbf{c},\textbf{d}) The uneven probe intensity distribution of the cavities, observed by an infrared CCD camera when the pump laser is off.  (\textbf{e}) Normalized transmission (NT) spectrum for the probe resonances, which correspond to the orange resonances shown in fig. \hyperref[fig:fig2main]{\ref{fig:fig2main}b}. The red (blue) dashed line corresponds to the probe wavelength region for probing the $L$ ($R$) OMO, as illustrated in (a,b). (\textbf{f}) The red (blue) curve is the $L$ ($R$) cavity probe transmission RF spectrum, when the pump is in the asynchronous region $- 0.13 < \Delta {\omega _L}/2\pi  <  - 0.10 $ GHz shown in fig. \hyperref[fig:fig3main]{\ref{fig:fig3main}d}; a strong peak at $f_R$ is observed but with very different amplitude for two probing conditions. The right inset figures show the same curves in linear scale, emphasising the large difference between the blue and red curves. (\textbf{g}) Same curves shown in (f) but with the pump laser in the synchronous region $\Delta {\omega _L}/2\pi < -0.13$~GHz of fig. \hyperref[fig:fig3main]{\ref{fig:fig3main}d}. Here both cavities have similar amplitude at $f_S$, which can be clearly noticed in the linear scale inset.}
\label{fig:fig4main}
\end{center}
\end{figure*}
We experimentally verify that both structures are oscillating at the synchronized frequency by probing the mechanical oscillation of each cavity individually. This verifies that the amplitude death of one of the oscillators does not occur, a known phenomenon in coupled nonlinear oscillators~\cite{MirStr9007,YamShi84}. Note that based solely on the transmitted pump signal, which provides global information of the coupled OMO system, one cannot clearly distinguish the individual contribution from each OMO to the synchronized signal. Using a weak probe laser, as shown in the setup in figure \hyperref[fig:fig2main]{\ref{fig:fig2main}a}, we excite optical resonances that are not strongly coupled between the two OMOs and therefore selectively probe the oscillation of cavity $L$ or $R$. Due to their low optical quality factor ($Q_{opt} \approx 4 \times {10^4}$), probing these resonances also minimize perturbations to the mechanical oscillations. figure \hyperref[fig:fig4main]{\ref{fig:fig4main}e} shows the transmission of the probe mode where an asymmetric splitting is evident. This asymmetry is due to the difference between the optical resonant frequencies of the $L$ and $R$ OMO at the probe wavelength. The uneven light intensity distribution in the two OMOs due to this mode asymmetry can be directly observed by capturing the scattered light with an infrared camera (fig. \hyperref[fig:fig4main]{\ref{fig:fig4main}c,d}). We probe the OMOs in two pump conditions: between the 1st and 2nd Hopf bifurcation, and after the 2nd Hopf bifurcation for ${P_{in}} =(11\pm1)$~\textmu W , indicated by the white lines in figure \hyperref[fig:fig3main]{\ref{fig:fig3main}d}. When the pump laser is in the range $- 0.13 < \Delta {\omega _L}/2\pi  <  - 0.10 $  GHz (between the dashed and solid line in fig. \hyperref[fig:fig3main]{\ref{fig:fig3main}d}), we expect that only the $L$ OMO to oscillate. Indeed, the probe laser RF spectrum shows a strong peak at ${f_L}$ (red curve in fig. \hyperref[fig:fig4main]{\ref{fig:fig4main}f}). This same peak does show in the spectrum when probing the $R$ OMO (blue curve in fig. \hyperref[fig:fig4main]{\ref{fig:fig4main}f}) but it is 13 dB weaker. These results confirm that in this range, the oscillation state is indeed asynchronous and the $L$ OMO oscillates with much larger amplitude. When the pump laser is in the range $\Delta {\omega _L}/2\pi  <  - 0.13$ GHz we expect from figure \hyperref[fig:fig3main]{\ref{fig:fig3main}d} the cavities to be synchronized and the optical probe signal to have an RF tone of similar amplitude at the synchronized frequency ${f_S}$ when probing individually the $L$ and $R$ OMOs. Indeed when the two OMOs are individually probed (blue and red curves in fig. \hyperref[fig:fig4main]{\ref{fig:fig4main}g}), the RF peaks at the synchronized frequency ${f_S}$ differs in amplitude by less than 0.5 dB. This shows that both cavities are indeed oscillating at the synchronized frequency. 

We have demonstrated the onset of synchronization of two optomechanical oscillators coupled through the optical radiation field. Monolithic integration and the ability to control the coupling strength are promising for realizing large oscillator networks in which the oscillators can be addressed individually. Furthermore, established and future micro-photonics techniques such as electro-optic and thermo-optic techniques can now be extended to switch, filter and phase shift the coupling of these oscillators. Here we demonstrated coupling the near field between oscillators which can be switched on and off by thermo-optical means. In order to achieve long range coupling of mechanical oscillators, optical waveguides and optical fibres could be used enabling oscillator networks spread over large areas only limited by optical waveguide/fibre losses. Optically mediated mechanical coupling will also remove the restrictions of neighbourhood while creating 1D/2D/3D mechanical oscillator arrays ~\cite{ArlMyeRou1104}. Using long range, directional and controllable mechanical coupling, synchronized optomechanical systems may enable a new class of devices in sensing, signal processing and on-chip non-linear dynamical systems~\cite{Mar1110}.

